NewsStand CoronaViz: A Map Query Interface for Spatio-Temporal and Spatio-Textual Monitoring of Disease Spread

With the rapid continuing spread of COVID-19, it is clearly important to be able to track the progress of the virus over time in order to be better prepared to anticipate its emergence and spread in new regions as well as declines in its presence in regions thereby leading to or justifying "reopening" decisions. There are many applications and web sites that monitor officially released numbers of cases which are likely to be the most accurate methods for tracking the progress of the virus; however, they will not necessarily paint a complete picture. To begin filling any gaps in official reports, we have developed the NewsStand CoronaViz web application (https://coronaviz.umiacs.io) that can run on desktops and mobile devices that allows users to explore the geographic spread in discussions about the virus through analysis of keyword prevalence in geotagged news articles and tweets in relation to the real spread of the virus as measured by confirmed case numbers reported by the appropriate authorities. NewsStand CoronaViz users have access to dynamic variants of the disease-related variables corresponding to the numbers of confirmed cases, active cases, deaths, and recoveries (where they are provided) via a map query interface. It has the ability to step forward and backward in time using both a variety of temporal window sizes (day, week, month, or combinations thereof) in addition to user-defined varying spatial window sizes specified by direct manipulation actions (e.g., pan, zoom, and hover) as well as textually (e.g., by the name of the containing country, state or province, or county as well as textually-specified spatially-adjacent combinations thereof), and finally by the amount of spatio-temporally-varying news and tweet volume involving COVID-19.

==> Makefile <==
MAIN = corona_tracking

all: $(MAIN).pdf

define GNUPLOT_FIG =
plots/$(1)_$(2).tex: plots/plot_data.gnuplot
	cd plots ; gnuplot -e "$(2)='true'" -e "data='$(1)'" plot_data.gnuplot
endef

GNUPLOT_FIGURES = us washington hubei cn world
$(foreach fig,$(GNUPLOT_FIGURES),$(eval $(call GNUPLOT_FIG,$(fig),filter)))
$(foreach fig,$(GNUPLOT_FIGURES),$(eval $(call GNUPLOT_FIG,$(fig),nofilter)))
$(eval $(call GNUPLOT_FIG,world,twitter))
$(eval $(call GNUPLOT_FIG,us,twitter))

$(MAIN).pdf : $(MAIN).tex $(MAIN).bib application_screenshot.png\
	$(addprefix plots/,$(addsuffix _filter.tex,$(GNUPLOT_FIGURES)))\
	$(addprefix plots/,$(addsuffix _nofilter.tex,$(GNUPLOT_FIGURES)))\
	plots/world_twitter.tex plots/us_twitter.tex
	(. /usr/share/Modules/init/sh &&\
	module load texlive/2018) ;\
	pdflatex -draftmode $(MAIN) &&\
	bibtex $(MAIN) &&\
	pdflatex -draftmode $(MAIN) &&\
	pdflatex $(MAIN)

fast: $(MAIN.tex)
	(. /usr/share/Modules/init/sh &&\
	module load texlive/2018) ;\
	pdflatex $(MAIN)

clean:
	rm -rf $(MAIN).{pdf,aux,bbl,log,blg,out} plots/*{.eps,.tex,-eps-converted-to.pdf}


==> corona-queries.tex <==
\begin{document}

\section{Queries}

The values of all of the variables in NewsStand CoronaViz are
presented in a time-varying manner as time moves on with the aid
of a time slider thereby leading them to be characterized as
{\em dynamic} variables.  This is in contrast to conventional 
visualization tools where such variables are presented in a graph
where time is the horizontal axis and the variable value is the
vertical axis thereby leading them to be characterized as
{\em static}.  Thus we see that the presentation manner is the 
key to the characterization.
It is not easy to present several static variables as they tend
to clutter the display regardless of whether they are represented
as one graph for the set of all variables or one graph per variable.
The situation becomes more complex when values of the variables vary in
a spatially-varying manner.  In this case the only way to deal with
the static variables is to repeat the graph at each location.
This is OK when the data is spatially sparse but this is not something
we can count on.

In contrast, NewsStand CoronaViz deals with variables that are both
time-varying and spatially varying by re-examining the dimensionality
of the data in the sense that a time slider is a natural
representation of one-dimensional data (i.e., time) while a
two-dimensional map is a natural representation of two-dimensional
data.  The problem is how we we represent the values of the variables.
One possible solution is via a histogram but this leads to clutter
on the display and is cumbersome when the data is not spatially
sparse.  Moreover, there may be a layout problem here in the sense
that we cannot allow the histograms to overlap.  An alternative
common solution with the same overlap issues is to use solid
concentric circles where the radii of the circles correspond to the
value and the color corresponds to the identity of the variable.  The
problem here is when we has multiple dynamic variables as 
we do, then only the one with the largest magnitude can be viewed.
One solution is to vary the colors of the circles but if this method
is used, then we must pay close attention to the order in which we
display the circles so that the one with the largest radius is
displayed first and the remaining circles be displayed in decreasing
order of radius values (this is analogous to the ``back-to-front"
z-buffer display algorithm used in computer graphics).  
We can avoid the need to worry about the order in which we display
the circles by using hollow concentric circles where again the color
indicates the identity of the variable while the radius corresponds to
a scaled variable magnitude value.  We use the term {\em geo-circle}
to describe this approach which

The visual strain posed by having a large number of circles can be
relieved by drawing the circles using broken lines of the same width.
At times, the width of the broken lines can be increased with the goal
of drawing attention to a particular set of concentric circles (i.e., a
location whose variable values at a particular instance of time) which
is of interest. We do this in the case of a hover operation wile
panning on the map to show the spatially closest location with nonzero 
variable values.  This operation is common in computer graphics where
it is known as a ``pick'' operation (e.g.,
see~\cite{Foley-and-VanDam}). 

NewsStand CoronaViz makes use of 6 dynamic variables comparing the
number of confirmed cases. active cases, recoveries (although not
reported by all jurisdictions), and deaths, and also the
number of news articles and tweets that mention Coronavirus.
Concentric circles (i.e., geo-circles) are used for 4 disease related
variable values while concentric solid circles with different colors,
depending on the number of documents and the nature of the document.
It is advised to just display one of the news articles or tweets
variables in which the count is displayed in the circle.  Otherwise
no count is displayed.

The concentric circles make is easy to spot trends and similar values
on the map by looking at the magnitude of the radii.  Other observations
of interest involve trends such as noting lower confirmed case and 
death counts over time as the circles get smaller.  Another
encouraging trend is when confirmed case counts become smaller than death counts,
In essence, we are speaking about when concentric circles intersect
and change their relative order.  Of course this must be treated
with caution as the magnitudes of the variables change).

There are a number of ways of presenting the variable values.  The
default in our case is of a cumulative nature.  However, it is
possible to normalize the values over population, or even area.
Normalizing over the area is of possible interest as it could be
used to see if densely populated areas are more likely to lead to
higher incidences of COVID-19 and deaths.

Our goal is to endow NewsStand CoronaViz with a full compliment
of queries that are consistent with its role as a spatio-temporal
and spatio-textual database.  First of all, we have two types of
queries:
\begin{enumerate}
\item location-based:  given a location, what features are present
as well as what are the values of certain variables.  In the
case of documents, we are looking for documents that mention
a particular location name.
\item feature-based:  given a feature, where is it located.
This is also known as spatial data mining.
For example, given a tweet or a news article, what locations
does it mention.  In NewsStand CoronaViz we might be looking for
locations where there are no deaths.
\end{enumerate}

The location-based queries are supported by the ability to pan the
map with a hover operation and always returning the variable values
with the nearest location for which we have data.
NewsStand CoronaViz supports this query by a PR quadtree where we
have one PR quadtree for each of the disease-related dynamic queries.
The feature-based queries are supported by the NewsStand and
TwitterStand databases that support the news and tweet 
document system.  Feature-based queries require the use of a
pyramid-like data structure on each of the disease-related dynamic
queries.

The animation window is a very important feature as it enables
the execution of a range query where the range is temporal.  Users
can vary the start and end times as well as the animation step size.
In addition users can specify what statistic is being computed
for the window.  It can be cumulative, a time instance like a daily,
weekly, monthly, or any period of days.  Average values for the
window can also be computed.  This is particularly useful for the
``reopen'' discussion which is often based on a rolling 
weekly daily average computation.

Spatial range (also known as window) queries are also of great
interest.  In this case, users use pan and zoom operations to
get a map that is focused on a particular spatial region (e.g.,
the minimum bounding areal box that contains Italy.
Not that in this case, there is also overlap with 
San Marino and the Holy See (i.e., the Vatican in Rome).  In this case
we display the values of the dynamic variables for all
three of these entities.  To get just the values for Italy, users
must zoom in further so that San Marino and the Holy See are not
in the window.  Alternatively if users only want Italy, then they
could simply pose the textual query for which an appropriate
index exists.  Note that as NewsStand Coronaviz zooms into a
region, it has access to more data (as low as county level data).
In the case of tweets and news articles, the area spanned
by the location for which we have this data is not necessarily
coincident with the location for which we have disease-related data
but they are close and thus we report the variable's values
over all the regions that overlap the region of the document related
location for which we have no data (e.g., Egypt and Libya for Benghazi).

Notice that NewsStand  CoronaViz enables the execution of the full
compliment of spatio-temporal queries as it supports keeping location
fixed while varying time via the time slider, keeping time fixed and
letting location vary via the hover, panning, and zooming operations.
We can also pick any range of time or space.  The full compliment of 
spatio-textual queries is possible as users can simply go to a
location on the map and obtain the relevant documents, while also
being able to ask for all documents mentioning a particular
keyword.  They can also take advantage of spatial synonyms
when they don't know the exact name of the location of interest.
For example, when seeking a ``Rock Concert in Manhattan,'' concerts in
Harlem, New York City, and Brooklyn are all good answers because
of being contained in Manhattan, containing Manhattan, and being a
spatially adjacent borough, respectively.  This is an example
of a proximity query which we saw previously via the use of a hover
operation in the case of spatial proximity, and the time slider 
in the case of temporal proximity.  Note that in the case of 
temporal proximity, we provide the capability to halt an animation at
arbitrary time instances as well as resuming or terminating it.
In addition, users are also able to set the speed of the animation,
as well as to step through an animation very x time units both
forward and backward in time.



==> plots/us_twitter.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4752.00,3484.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(946,1013){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(946,1294){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(946,1576){\makebox(0,0)[r]{\strut{}$2000$}}%
      \put(946,1857){\makebox(0,0)[r]{\strut{}$3000$}}%
      \put(946,2138){\makebox(0,0)[r]{\strut{}$4000$}}%
      \put(946,2419){\makebox(0,0)[r]{\strut{}$5000$}}%
      \put(946,2701){\makebox(0,0)[r]{\strut{}$6000$}}%
      \put(946,2982){\makebox(0,0)[r]{\strut{}$7000$}}%
      \put(946,3263){\makebox(0,0)[r]{\strut{}$8000$}}%
      \put(1078,818){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}01/09}}}%
      \put(1439,818){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}01/23}}}%
      \put(1801,818){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}02/06}}}%
      \put(2162,818){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}02/20}}}%
      \put(2523,818){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}03/05}}}%
      \put(2884,818){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}03/19}}}%
      \put(3246,818){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}04/02}}}%
      \put(3607,818){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}04/16}}}%
      \put(3739,1013){\makebox(0,0)[l]{\strut{}$0$}}%
      \put(3739,1463){\makebox(0,0)[l]{\strut{}$5$}}%
      \put(3739,1913){\makebox(0,0)[l]{\strut{}$10$}}%
      \put(3739,2363){\makebox(0,0)[l]{\strut{}$15$}}%
      \put(3739,2813){\makebox(0,0)[l]{\strut{}$20$}}%
      \put(3739,3263){\makebox(0,0)[l]{\strut{}$25$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(209,2138){\rotatebox{-270}{\makebox(0,0){\strut{}Confirmed Cases}}}%
      \put(4245,2138){\rotatebox{-270}{\makebox(0,0){\strut{}Tweet Count}}}%
      \put(2342,154){\makebox(0,0){\strut{}Day and Month (2020)}}%
      \csname LTb\endcsname%%
      \put(2398,3090){\makebox(0,0)[r]{\strut{}Confirmed}}%
      \csname LTb\endcsname%%
      \put(2398,2870){\makebox(0,0)[r]{\strut{}Article}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{us_twitter-eps-converted-to}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plots/world_twitter.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4752.00,3484.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1078,1013){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(1078,1334){\makebox(0,0)[r]{\strut{}$5000$}}%
      \put(1078,1656){\makebox(0,0)[r]{\strut{}$10000$}}%
      \put(1078,1977){\makebox(0,0)[r]{\strut{}$15000$}}%
      \put(1078,2299){\makebox(0,0)[r]{\strut{}$20000$}}%
      \put(1078,2620){\makebox(0,0)[r]{\strut{}$25000$}}%
      \put(1078,2942){\makebox(0,0)[r]{\strut{}$30000$}}%
      \put(1078,3263){\makebox(0,0)[r]{\strut{}$35000$}}%
      \put(1210,818){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}01/09}}}%
      \put(1552,818){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}01/23}}}%
      \put(1895,818){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}02/06}}}%
      \put(2237,818){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}02/20}}}%
      \put(2580,818){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}03/05}}}%
      \put(2922,818){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}03/19}}}%
      \put(3265,818){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}04/02}}}%
      \put(3607,818){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}04/16}}}%
      \put(3739,1013){\makebox(0,0)[l]{\strut{}$0$}}%
      \put(3739,1294){\makebox(0,0)[l]{\strut{}$10$}}%
      \put(3739,1576){\makebox(0,0)[l]{\strut{}$20$}}%
      \put(3739,1857){\makebox(0,0)[l]{\strut{}$30$}}%
      \put(3739,2138){\makebox(0,0)[l]{\strut{}$40$}}%
      \put(3739,2419){\makebox(0,0)[l]{\strut{}$50$}}%
      \put(3739,2701){\makebox(0,0)[l]{\strut{}$60$}}%
      \put(3739,2982){\makebox(0,0)[l]{\strut{}$70$}}%
      \put(3739,3263){\makebox(0,0)[l]{\strut{}$80$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(209,2138){\rotatebox{-270}{\makebox(0,0){\strut{}Confirmed Cases}}}%
      \put(4245,2138){\rotatebox{-270}{\makebox(0,0){\strut{}Tweet Count}}}%
      \put(2408,154){\makebox(0,0){\strut{}Day and Month (2020)}}%
      \csname LTb\endcsname%%
      \put(2530,3090){\makebox(0,0)[r]{\strut{}Confirmed}}%
      \csname LTb\endcsname%%
      \put(2530,2870){\makebox(0,0)[r]{\strut{}Article}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{world_twitter-eps-converted-to}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> temp.tex <==
\section{Queries}

The values of all of the variables in NewsStand CoronaViz are
presented in a time-varying manner as time moves on with the aid
of a time slider thereby leading them to be characterized as
{\em dynamic} variables.  This is in contrast to 
visualization tools where such variables are presented in a graph
where time is the horizontal axis and the variable value is the
vertical axis thereby leading them to be characterized as
{\em static}.  Thus we see that the presentation manner is the
key to the characterization.
It is not easy to present several static variables as they tend
to clutter the display regardless of whether they are represented
as one graph for the set of all variables or one graph per variable.
The situation becomes more complex when values of the variables vary in
a spatially-varying manner.  In this case the only way to deal with
the static variables is to repeat the graph at each location.
This is OK when the data is spatially sparse but this is not something
we can count on.

In contrast, NewsStand CoronaViz deals with variables that are both
time-varying and spatially varying by re-examining the dimensionality
of the data in the sense that a time slider is a natural
representation of one-dimensional data (i.e., time) while a
two-dimensional map is a natural representation of two-dimensional
data.  The problem is how we we represent the values of the variables.
One possible solution is via a histogram but this leads to clutter
on the display and is cumbersome when the data is not spatially
sparse.  Moreover, there may be a layout problem here in the sense
that we cannot allow the histograms to overlap.  An alternative
common solution with the same overlap issues is to use solid
concentric circles where the radii of the circles correspond to the
value and the color corresponds to the identity of the variable.
This type of visualization is known in cartography as a proportional
symbol map~\cite{slocum_thematic_2009}. The 
problem here is when we have multiple dynamic variables as
is the case for our application, then only the one with the largest magnitude can be viewed.
One solution is to vary the colors of the circles but if this method
is used, then we must pay close attention to the order in which we
display the circles so that the one with the largest radius is
displayed first and the remaining circles be displayed in decreasing
order of radius values (this is analogous to the ``back-to-front''
z-buffer display algorithm used in computer graphics).
We can avoid the need to worry about the order in which we display
the circles by using hollow concentric circles where again the color
indicates the identity of the variable while the radius corresponds to
a scaled variable magnitude value.  We use the term {\em geo-circle}
to describe this approach.

The visual strain posed by having a large number of circles can be
relieved by drawing the circles using broken lines of the same width.
At times, the width of the broken lines can be increased with the goal
of drawing attention to a particular set of concentric circles (i.e., a
location whose variable values at a particular instance of time) which
is of interest. We do this in the case of a hover operation wile
panning on the map to show the spatially closest location with nonzero
variable values.  This operation is common in computer graphics where
it is known as a ``pick'' operation (e.g.,
see~\cite{Fole90}).

NewsStand CoronaViz makes use of 6 dynamic variables comparing the
number of confirmed cases. Active cases, recoveries (although not
reported by all jurisdictions), and deaths, and also the
number of news articles and tweets that mention Coronavirus.
Concentric circles (i.e., geo-circles) are used for 4 disease related
variable values while concentric solid circles with different colors,
depending on the number of documents and the nature of the document.
It is advised to just display one of the news article or tweet
variables in which the count is displayed in the circle.  Otherwise
no count is displayed.

The concentric circles make is easy to spot trends and similar values
on the map by looking at the magnitude of the radii.  Other observations
of interest involve trends such as noting lower confirmed case and
death counts over time as the circles get smaller.  Another
encouraging trend is when confirmed case counts become smaller than death counts,
In essence, we are speaking about when concentric circles intersect
and change their relative order.  Of course this must be treated
with caution as the magnitudes of the variables change).

There are a number of ways of presenting the variable values.  The
default in our case is of a cumulative nature.  However, it is
possible to normalize the values over population, or even area.
Normalizing over the area is of possible interest as it could be
used to see if densely populated areas are more likely to lead to
higher incidences of COVID-19 and deaths.

Our goal is to endow NewsStand CoronaViz with a full compliment
of queries that are consistent with its role as a spatio-temporal
and spatio-textual database.  First of all, we have two types of
queries:
\begin{enumerate}
\tightlist
\item location-based:  given a location, what features are present
as well as what are the values of certain variables.  In the
case of documents, we are looking for documents that mention
a particular location name.
\item feature-based:  given a feature, where is it located.
This is also known as spatial data mining.
For example, given a tweet or a news article, what locations
does it mention.  In NewsStand CoronaViz we might be looking for
locations where there are no deaths.
\end{enumerate}

The location-based queries are supported by the ability to pan the
map with a hover operation and always returning the variable values
with the nearest location for which we have data.
%NewsStand CoronaViz supports this query by a PR quadtree where we
%have one PR quadtree for each of the disease-related dynamic queries.
The feature-based queries are supported by the NewsStand and
TwitterStand databases that support the news and tweet 
document system.  Feature-based queries require the use of a
pyramid-like data structure on each of the disease-related dynamic
queries.

The animation window is a very important feature as it enables
the execution of a range query where the range is temporal.  Users
can vary the start and end times as well as the animation step size.
In addition users can specify what statistic is being computed
for the window.  It can be cumulative, a time instance like a daily,
weekly, monthly, or any period of days.  Average values for the
window can also be computed.  This is particularly useful for the
``reopen'' discussion which is often based on a rolling 
weekly daily average computation.

Spatial range (also known as window) queries are also of great
interest.  In this case, users use pan and zoom operations to
get a map that is focused on a particular spatial region (e.g.,
the minimum bounding areal box that contains Italy.
Not that in this case, there is also overlap with 
San Marino and the Holy See (i.e., the Vatican in Rome).  In this case
we display the values of the dynamic variables for all
three of these entities.  To get just the values for Italy, users
must zoom in further so that San Marino and the Holy See are not
in the window.  Alternatively if users only want Italy, then they
could simply pose the textual query for which an appropriate
index exists.  Note that as NewsStand Coronaviz zooms into a
region, it has access to more data (as low as county level data).
In the case of tweets and news articles, the area spanned
by the location for which we have this data is not necessarily
coincident with the location for which we have disease-related data
but they are close and thus we report the variable's values
over all the regions that overlap the region of the document related
location for which we have no data (e.g., Egypt and Libya for Benghazi).

Notice that NewsStand  CoronaViz enables the execution of the full
compliment of spatio-temporal queries as it supports keeping location
fixed while varying time via the time slider, keeping time fixed and
letting location vary via the hover, panning, and zooming operations.
We can also pick any range of time or space.  The full compliment of 
spatio-textual queries is possible as users can simply go to a
location on the map and obtain the relevant documents, while also
being able to ask for all documents mentioning a particular
keyword.  They can also take advantage of spatial synonyms
when they don't know the exact name of the location of interest.
For example, when seeking a ``Rock Concert in Manhattan,'' concerts in
Harlem, New York City, and Brooklyn are all good answers because
of being contained in Manhattan, containing Manhattan, and being a
spatially adjacent borough, respectively.  This is an example
of a proximity query which we saw previously via the use of a hover
operation in the case of spatial proximity, and the time slider 
in the case of temporal proximity.  Note that in the case of 
temporal proximity, we provide the capability to halt an animation at
arbitrary time instances as well as resuming or terminating it.
In addition, users are also able to set the speed of the animation,
as well as to step through an animation very x time units both
forward and backward in time.



